CAMEO: A Causal Transfer Learning Approach for Performance Optimization of Configurable Computer Systems

Modern computer systems are highly configurable, with hundreds of configuration options that interact, resulting in an enormous configuration space. As a result, optimizing performance goals (e.g., latency) in such systems is challenging due to frequent uncertainties in their environments (e.g., workload fluctuations). Recently, transfer learning has been applied to address this problem by reusing knowledge from configuration measurements from the source environments, where it is cheaper to intervene than the target environment, where any intervention is costly or impossible. Recent empirical research showed that statistical models can perform poorly when the deployment environment changes because the behavior of certain variables in the models can change dramatically from source to target. To address this issue, we propose CAMEO, a method that identifies invariant causal predictors under environmental changes, allowing the optimization process to operate in a reduced search space, leading to faster optimization of system performance. We demonstrate significant performance improvements over state-of-the-art optimization methods in MLperf deep learning systems, a video analytics pipeline, and a database system.

==> background.tex <==
\section{Background and Problem Statement}
\label{background}
% Predicting unknown values based on observed data is a problem central to many sciences, and well studied in statistics and machine learning. This problem becomes significantly harder if the training and test data do not have the same distribution,  for example because they come from different domains. Such a distribution shift can happen whenever the circumstances under which the training data were gathered are different from those for which the predictions are to be made. A rich literature exists on this problem of domain adaptation, a particular task in the field of transfer learning. 

% When the environment changes, a distribution shift can happen as the underlying data generating process may be different. These types of changes are fairly common in the systems' world i.e., software change, hardware change, workload change.
% In this section, we introduce the relevant definitions and the problem formulation.
\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{Figures/overview_cameo.pdf}
\caption{\small{Overview of \ourapproach}}
\label{fig:overview}
\end{figure*}
\subsection{Definitions}
% \paragraph{Performance Prediction Task.} \textit{We are given data for a single source domain $e_s$ and a single target domain $e_t$. Assume that the source domain data $(\mathcal{X}_{e_{s}},\mathcal{Y}_{e_{s}})$ is complete (i.e., no missing values). In the target domain, we only have access to a small subset of performance distribution data $(\mathcal{X}_{e_{t}}, \mathcal{Y}_{e_{t}})$. The task is to predict
% the missing values of the target variable $\mathcal{Y}_{e_{t}}$ given the available source and target domain data without any additional interventions in the target $e_t$.}

% \paragraph{Task 2 (Performance Debugging Task).} \textit{We are given data for a single source domain $e_s$ and a single target domain $e_t$. Assume that the source domain data $(\mathcal{X}_{e_{s}},\mathcal{Y}_{e_{s}})$ is complete (i.e., no missing values). In the target domain, we only have access to a sample $\mathcal{X}_{e_{t}}$, its corresponding tail response value $\mathcal{Y}_{e_{t}}$, an expected response value $\mathcal{Y}^{\dagger}_{e_{t}}$ and a budget $\mathcal{B}$ if additional observations are needed. The task is to find $\mathcal{X}^{\ast}_{e_{t}}$ for which the corresponding response value $\mathcal{Y}^{\ast}_{e_{t}} \geq \mathcal{Y}^{\dagger}_{e_{t}}$ given the available source and target domain data without some additional interventions in the target $e_t$ within budget $\mathcal{B}$.}
\noindent \textbf{Configuration Space $\mathcal{O}$. }
Let $\mathcal{O}_i$ indicate the $i^{th}$ configuration option of a system, which can be set to a range of different values (e.g., categorical, boolean, and numerical). The configuration space
is a Cartesian product of all options $\mathcal{O} = Dom(\mathcal{O}_1) \times ... \times Dom(\mathcal{O}_d$), where d is the number of options. A configuration $o$ is then a member of the configuration space $\mathcal{O}$ in which all options are set to a given value within the range of permitted values for that option.

\noindent \textbf{Environment Space $\mathcal{E}$.} We describe an environment $e$ drawn from a given environment space $\mathcal{E}$ which consists of possible combinations of hardware, workload, software and deployment topology. 

\noindent \textbf{Causal Performance Model $\mathcal{G}$.}
% ~\rayb{can we give a picture of CPM?}
A causal performance model (CPM), denoted by $\mathcal{G}$, is an acyclic directed mixed graph (ADMG) that provides the functional dependencies (e.g., how variations in one or multiple variables determine variations in other variables) between configuration options, system events, and performance objectives. While interpreting a CPM, we view the nodes as variables and the arrows as causal connections.

\noindent \textbf{Observation.}
In the \textit{observational} formulation, we measure the distribution of an outcome variable (e.g., \textsf{latency} $\mathcal{Y}$) given that we \textit{observe} another variable (e.g., \textsf{cpu frequency} $\mathcal{O}_{i}$ for $1 \leq i 
\leq d$) taking a certain value $o_i$ (e.g., $\mathcal{O}_{i}= o_i$), denoted by $Pr(\mathcal{Y}~|~\mathcal{O}_{i}= o_i)$. 
%This is a familiar expression that, given adequate data, modern supervised machine learning algorithms can estimate.

\noindent \textbf{Intervention.} The \textit{interventional} inference tackles a harder task of estimating the  effects of deliberate actions. For example, we measure how the distribution of an outcome (e.g., \textsf{latency} $\mathcal{Y}$) would change if we (artificially) intervened during the data gathering process by forcing the variable \textsf{cpu frequency} $\mathcal{O}_{i}$ to a certain value $o_i$, but otherwise retain the other variables (e.g., \textsf{dirty ratio}) as is. We can estimate the outcome of the artificial intervention by modifying the CPM to reflect our intervention and applying Pearl's \emph{do-calculus}~\cite{pearl2009causality} which is denoted by $Pr(\mathcal{Y}~|~do(\mathcal{O}_{i}= o_i))$. Unlike observations, there is a structural change of CPM due to intervention that goes along with a change of probability distribution over the variables.

% This is done by building a causal performance model and modifying them to reflect our intervention. Then, using the modified causal graph and \textit{do-causal calculus} rules~\cite{pearl2009causality} we may estimate the outcome of the artificial intervention. This process is computationally efficient since we reason over existing data instead of gathering additional measurements.


% A CPM has several constraints such as (i) not every variables can be intervened (e.g., performance objectives and some system events cannot be intervened) (ii) configuration options are independent and do not have a causal relation between them. Note that such constraints enable incorporating domain knowledge and enable further sparsity that facilitates learning with low sample sizes.

% \noindent \textbf{Surrogate Model} A surrogate models is used to approximate the performance objective to optimize, which is usually computationally expensive to evaluate and not available in closed form. Surrogate models are trained with evaluations of a small number of subset of the configuration space $\mathcal{O}$ and are used to predict the objective functions value using
% $\hat{\mathcal{Y}}(o)=\mu(O)$ with estimation uncertainty $\sigma(o)$ for each configuration $o \in \mathcal{O}$. 

\noindent \textbf{Bayesian Optimization.} 
Bayesian Optimization (BO) is an efficient framework to solve global optimization problems using black-box evaluations of expensive performance objectives $\mathcal{Y}$. A typical BO approach consists two main elements: the surrogate model and the acquisition function. The surrogate models are trained with a small number of configuration measurements and are used to predict the objective functions value $\hat{\mathcal{Y}} = f(o)$ using predictive mean $\mu(o)$ and uncertainty $\sigma(o)$ for configurations $o \in \mathcal{O}$. A common practice is to use Gaussian processes (GPs) as surrogate model where the GP distribution over $f(o)$ is fully specified by its mean function its mean function $\mu(o)$  and its covariance function $k_c(o,o')$. The kernel or covariance function $k_c$ captures the regularity in the form of the correlation of the marginal distributions $f(o)$ and $f(o')$. After the surrogate model outputs predictive mean and uncertainty for the unseen configurations, \ourapproach needs an acquisition function to select the best configuration to sample. A good acquisition function should balance the trade-offs between exploration and exploitation. 


% The three essential elements of the Bayesian optimization framework are:
% \paragraph{\textbf{2.1.} Surrogate Model.} Surrogate models replace expensive, time-consuming, and otherwise difficult to measure black-box functions with models that provide an approximation of the measurements from the underlying black-box process and are inexpensive to evaluate.

% \noindent \textbf{Acquisition Function.} This is used to score the utility of evaluating a candidate configuration $o \in \mathcal{O}$ based on the statistical model that is a cheap alternative of the expensive performance objective function. 

% Some popular acquisition functions in the SOBO literature include expected improvement (EI)~\shortcite{emmerich2008computation}, upper confidence bound (UCB)~\shortcite{srinivas2012information}, predictive entropy search (PES)~\shortcite{hernandez2014predictive}, and max-value entropy search (MES)~\shortcite{wang2017max}. 


\subsection{Problem Formulation}

Let us consider a highly configurable system of interest with configuration space ${\mathcal{O}}$, system events and performance counters space $\mathcal{C}$, and a performance objective  $\mathcal{Y}$.
%, that are observed in different environments $e \in \bm{\mathcal{E}}$. 
Configuration options and system events are jointly represented as a vector %$\mathcal{X}=(\mathcal{O},\mathcal{S})=(\mathcal{O}_{{1}},...,\mathcal{O}_{{d}},\mathcal{S}_{{1}},...,\mathcal{S}_{{l}})$, where $d\geq 1$ and $l\geq 1$. 
$\mathcal{X}=(\mathcal{O},\mathcal{C})$.
We assume that in each environment $e \in \mathcal{E}$, the variables $(\mathcal{X}_e,\mathcal{Y}_e)$ have a joint distribution $\mathcal{P}_e$. In the source environment, there are no budget constraints and data are i.i.d, yielding $n$ observations. In the target environment, $m$ ($\ll n$) observations can be collected within a given budget $\mathcal{B}$. When we are given data for a source domain $e_{\text{s}}$, a smaller number of initial samples in the target domain $e_{\text{t}}$, and a budget $\mathcal{B}$,
%(we assume that the source domain data $(\mathcal{X}_{e_{s}},\mathcal{Y}_{e_{s}})$ is complete,e.g, no missing values). 
the task is to find a configuration $o$ that minimizes the performance objective $y$ in the target $e_{\text{t}}$ using: 
\begin{equation}
    \text{argmin}_{o \in \mathcal{O}} \mathcal{Y}_{{e}_\text{t}} \ \text{within} \ \mathcal{\beta} \ \text{in} \ e_{\text{t}}
\end{equation}
Note in \Cref{methodology}, construction of a causal performance model uses all the variables while the causal Gaussian processes only search through the configurations as we cannot control system events.



% \paragraph{Task 4 (Performance Planning Task).} \textit{We are given data for a single source domain $e_s$ and a single target domain $e_t$. Assume that the source domain data $(\mathcal{X}_{e_{s}},\mathcal{Y}_{e_{s}})$ is complete (i.e., no missing values). In the target domain, we only have an expected response value $\mathcal{Y}^{\dagger}_{e_{t}}$. The task is to estimate the budget $\mathcal{B}$ required to determine $\mathcal{X}^{\ast}_{e_{t}}$ for which the corresponding response value $\mathcal{Y}^{\ast}_{e_{t}} \geq \mathcal{Y}^{\dagger}_{e_{t}}$ given the available source and target domain data without some additional interventions in the target $e_t$.}

==> intro_bck.tex <==
\section{Introduction}
\label{sec:intro}
Modern software systems continuously deployed in heterogeneous environments, such as public/private cloud, high-performance computing platforms, and system-on-chip (SoCs), are highly configurable across the software/hardware stack.
In these systems, optimizing the performance, e.g., latency and energy, is crucial for faster data processing, better user satisfaction, and lower application maintenance cost~\cite{wang2021morphling,ding2022cello}. One possible way to achieve these goals is to tune the systems with the optimal hardware and software configuration options. For instance, \textit{cpu frequency}, \textit{swappiness}, and \textit{memory growth} are exposed to developers such that they can configure both the system and applications to operate with optimal
%~\rayb{I am not sure whether latency is the right word here. It is not a particular latency that users hoped for, it is more like optimal one, right?}
latency~\cite{xu2015hey, colin2018reconfigurable, blocher2021switches}.





Selecting an optimal configuration in a highly configurable system, however, is challenging because: 
(i) Each component in the system stack, i.e., software,
%~\rayb{different software pieces in the software stack?}
hardware, OS, etc., has its configuration options that interact with each other, giving rise to a combinatorial configuration space~\cite{JC:MASCOTS16,wang2018understanding,halin2019test,velez2022study}, (ii) estimating the effect of configurations on performance is expensive as one needs to collect run-time behavior of the system for each configuration option, and (iii) unknown constraints exist among configuration options. 
Moreover, to meet growing user requirements and reduce service management costs, the underlying systems often undergo environmental changes, i.e., hardware updates, deployment topology change, etc.~\cite{ding2021generalizable}. Therefore, performance optimization of such evolving systems becomes even more challenging as there is no guarantee that the optimal configurations found in one environment will remain optimal in a different environment\footnote{we define an environment as a combination of hardware, workload, software, and deployment topology}. 



% \begin{figure}[t]
%   \subfloat[]{
% 	\begin{minipage}[c][1\width]{
% 	   0.46\linewidth}
% 	   \centering
% 	   \includegraphics[width=\textwidth]{Figures/dist_change_histogram.pdf}
% 	\end{minipage}}
%  \hfill 	
%   \subfloat[]{
% 	\begin{minipage}[c][1\width]{
% 	   0.46\linewidth}
% 	   \centering
% 	   \includegraphics[width=\textwidth]{Figures/simpsons.pdf}
% 	\end{minipage}}
% \caption{\small{(a) Optimal configuration for \textsc{MLPerf Object Detection} pipeline deployed on Jetson TX2 does not remain optimal on Jetson Xavier. (b) Statistical correlation-based approaches wrongly identify an inverse proportional correlation between \textsf{cache miss} and \textsf{latency}. However, when \textsf{EMC frequency} is used to group the data (as shown in ellipses), \textsf{latency} becomes proportional to a \textsf{cache miss}.
% %rely on spurious correlation and are incorrect. 
% %\rayb{b is not clear....correlation of what?}
% }}
%     \label{fig:hw_change_intro}
% \vspace{-6mm}
% \end{figure}
\smallskip
\noindent\textbf{Existing works and gap.} \textit{(i) Performance Optimization in Configurable Systems.} Several approaches have been proposed for performance optimization of configurable systems, e.g., Bayesian optimization (BO)~\cite{hutter2011sequential,yigitbasi2013towards,wu2015deep,alipourfard2017cherrypick,menon2020auto}, BO with regression~\cite{ding2022cello}, prediction models~\cite{chen2021efficient}, search space modification~\cite{hsu2018scout}, and online few-shot learning~\cite{blocher2021switches}. However, using these approaches in the target environment~\rayb{What is a target environment, first time appearing here} requires many queries which are too expensive to collect in the target environment. Using the optimal configuration found by these methods in a source environment~\rayb{Again, what is a source environment? I think we need to explain the source-target setting first before talking about the limitation} is also suboptimal as the optimal configuration in one environment usually no longer remains optimal in the other (see \Cref{fig:hw_change_intro} for an example).
%(as shown in Figure~\ref{fig:hw_change_intro} (a)).
%, and needs to be run from scratch. 
%Repeating the costly optimization process from scratch is not feasible, especially for systems deployed in production, because it would disrupt service availability and negatively impact user experience. 

\noindent\textit{(ii) Transfer Learning for Performance Modeling.} In real-world deployment scenarios, developers often have access to performance evaluations of different configurations from previous runs of the same system in other environments (e.g., a staging environment\footnote{A staging environment is a nearly exact replica of a production environment for software testing}).
%, i.e., staging~\rayb{What is staging? performance eval or previous traces?}. 
Exploiting such additional sources of information across environments
% (a key concept in \textit{transfer learning}) 
can result in efficient optimization, as demonstrated by recent work where transfer learning has been successfully applied to performance modeling of software systems~\cite{jamshidi2017transfer, jamshidi2018learning,krishna2019whence,iqbal_transfer_2019,martin2021transfer,lesoil2022transferring}. Such methods can be extended for performance optimization by building a search heuristic with summary statistics from the models. Zhang et al. \cite{zhang2021restune} proposed \restune which trained an ensemble model to represent prior knowledge from source environment and leveraged the extracted knowledge to speed up the performance optimization for a new task. 
% Hakhamaneshi et al. \cite{hakhamaneshi2021jumbo} proposed JUMBO, a multi-task BO method for optimization across environments. 
However, each environmental change can potentially incur a distribution shift. The underlying ML models used in these transfer learning methods are vulnerable to spurious correlations, which do not hold across distribution shifts and result in inferior performance ~\cite{zhou2021examining,ming2022impact,iqbal2022unicorn} (see \Cref{sec:motivation_causal} for a concrete example). 

% For example, our observational data for a \textsc{MLPerf object detection}~\cite{reddi2020mlperf} (MOD) pipeline deployed on different resource constrained edge devices (\textsc{TX2, TX1}, and \textsc{Xavier}) indicates that there is a distribution shift of varying intensity depending on the type of hardware changes that takes place (shown in Figure~\ref{fig:hw_change_intro} (a)). Thus, the ML-based approaches cannot be reliably reused as the independent and identically distributed (\textit{i.i.d}) assumption is violated~\cite{shen2021towards}.
% \begin{figure}[]
%     \centering
%      \includegraphics[width=0.5\columnwidth]{Figures/intro_hw_change.pdf}
%     \caption{An example of a \textsc{MLPerf Object Detection} pipeline. Here, the hardware is changed from Jetson TX2 to Jetson Xavier or TX1.}
%     \label{fig:deployment}
% \end{figure}

%\Cref{fig:hw_change_intro}(b) shows an example where the observational data indicates that \textit{cache miss} is negatively correlated with latency. Any ML model built on this data is likely to predict with high confidence that higher \textit{cache miss} leads to lower latency. However, this is counter-intuitive as higher \textit{cache miss} should, in theory, increase latency, but not decrease it. When we group data based on \textit{emc frequency}-a confounder variable~\footnote{confounder variable is a third variable that influences both the supposed cause (i.e., \textit{cache miss}) and the supposed effect (i.e., \textit{latency})}-we observe that within each group of \textit{emc frequency}, \textit{latency} increases as \textit{cache miss} increases. The presence of such confounder variables obfuscates an ML model's ability to identify the correct relationship. With thousands of configurations, inferring such nuanced information from ML-based approaches would require a considerable amount of measurements and extensive domain expertise, which is not practical, if not impossible. 
%As a result, ML-based approaches suffer from several shortcomings: (i) they become unreliable in unseen environments, and (ii) they are incorrect due to spurious correlations~\cite{zhou2021examining,ming2022impact,iqbal2022unicorn}(details in~\ref{sec:motivation}). 

\noindent\textit{(iii) Usage of Causal Analysis in Configurable Systems.} To address the problem of spurious correlations, recent work has leveraged causal inference \cite{pearl2009causal} to build a causal performance model\footnote{A causal performance model is an acyclic directed mixed graph, with nodes being variables and arrows being causal connections. It represents the dependencies (a.k.a. causal structures) among configuration options, system events, and performance objectives.} that captures the dependencies (a.k.a., causal structures) among configuration options, system events, and performance objectives. However, existing work mainly focuses on the setting of prediction \cite{iqbal2022unicorn}, which usually uses different underlying ML models (e.g., regression), than the problem of optimization. Besides, the causal graphs in the source and target can still have some differences (see \Cref{fig:graph_diff} for an example). Therefore, directly reusing the causal structure from the source can be problematic as well. 
%~\rayb{todo: rewrite this para.}

In summary, all these existing works are suboptimal for performance optimization when environment changes because: the knowledge extracted by these methods from the source ((i) optimal configuration) has changed and cannot be directly applied to the target, the model ((ii) ML based transfer learning model) used is limited to capture spurious correlations, or the model ((iii) causal model) is mostly stable but need further adaptation in the target environment.

\noindent\textbf{Our approach.}
The optimization approach should (i) use transfer learning to leverage the knowledge from both source and target, and (ii) use causal model to avoid spurious correlation. Consequently,
we propose \ourapproach (\textbf{Ca}usal \textbf{M}ulti \textbf{E}nvironment \textbf{O}ptimization), a causal transfer-based optimization
algorithm that aims to overcome
the limitation of prior approaches. Our approach builds on top of two previous work, JUMBO (a multi-task BO method) \cite{hakhamaneshi2021jumbo} and CBO (a causal BO method) \cite{causalBO} to satisfy all the three desired properties. A typical BO approach consists two main elements: the surrogate model and the acquisition function. The surrogate model tries to predict the performance objective when given a configuration and the acquisition function assigns a score to each configuration and choose the one with the highest score to query for the next iteration.
In \ourapproach, we first build two causal performance models to learn the dependency among configuration options, system events, and performance objectives for each environment using the previous performance measurements from the source environment and a considerably smaller number of measurements from the target environment. After that, we simultaneously train two Causal Gaussian Processes (CGPs) (which leverage the causal performance models when estimating means and variances) as two surrogate models: a warm-CGP in the source and a cold-CGP in the target.
% The use of CGPs in the entire framework ensures tractability in posterior inferences and updates. 
The acquisition function combines the individual acquisition functions of both CGPs such that the knowledge from both source and target is leveraged.
% It uses the warm-CGP to reduce the search space by filtering out a subset of configurations whose causal effect on the performance objective is limited. The acquisition function scores the remaining candidates for the cold-CGP to account for the imperfections in learning the feature space of warm-CGP, and the top candidate is queried. 
%.  Based on the several experimental pieces of evidence presented in the following sections, this paper proposes \ourapproach--a methodology that enables performance optimization of configurable system in a new environment that exploits knowledge learned from a previous environment with causal inference. \ourapproach first recovers the underlying causal structure from performance data. The causal performance model %instead of a performance model that has been learned using the mainstream regression-based approaches, 
% allows users to (i)~identify the root causes of performance faults, (ii)~estimate the causal effects of various configurable parameters on the performance objectives, and (iii)~prescribe candidate configurations to fix the performance fault or optimize system performance. 
% 
% we propose the use of causal models~\cite{pearl2000models, pearl2009causality} to express the complex interactions between the configurations and the performance objectives with a rich graphical representation. Then, using counterfactual reasoning~\cite{pearl2011algorithmization} we identify the root cause of non-functional faults and prescribe repairs to fix the misconfigured options.
% 
% The causal model would also highlight that other hidden factors (\eg, other processes running on the host) may affect the configurations (shown by \circled{?} in Fig.~\ref{fig:intro_fig}c). 
% 
% To this end, 
% 

% For example, in~\fig{intro_fig}, \ourapproach constructs a \textit{causal model} from observational data (as in Fig.~\ref{fig:intro_fig}c). This causal model indicates that \gpugrowth indirectly influences latency (via a \swapmem) and that the configuration options may be affected by certain other factors, \eg, resource manager allocating resources for other processes running on the host. \ourapproach uses counterfactual questions such as, ``what is the effect of \gpugrowth on latency if the available \swapmem was 2Gb?'' to diagnose the faults and recommend changes to the configuration options to mitigate these faults. 


\noindent\textbf{Evaluation.}~
We evaluated \ourapproach in terms of its \emph{effectiveness, sensitivity}, and \emph{scalability}, and compared it with five state-of-the-art performance optimization techniques (\smac~\cite{hutter2011sequential}, \restune and \restuner~\cite{zhang2021restune}, \cello~\cite{ding2022cello}, and \unicorn~\cite{iqbal2022unicorn}) using five real-world highly configurable systems (three \textsc{MLperf} pipelines (object detection, natural language processing, and speech recognition), a video analytics pipeline, and a database system) deployed on architecturally different edge devices and cloud under different environmental changes. Our results indicate that \ourapproach improves latency by 8.5\% and energy by 8.2\% on average than the best baseline optimization approach, \restuner.

\noindent \textbf{Contributions.}
Our contributions are the following: 
\begin{itemize}[noitemsep, nolistsep]
    \item We propose \ourapproach, a novel causal transfer-based approach that allows faster optimization of software systems when the environment changes. To the best of our knowledge, this is the first approach that addresses the performance optimization of the configurable system using transfer learning.
    %\item We study the key differences of performance behavior changes across environments to extract meaningful insights that can be utilized to design an effective search strategy for optimization.
    \item We conduct a comprehensive evaluation of \ourapproach by comparing it with three state-of-the-art optimization approaches on five real-world highly configurable systems under a range of different environmental changes and show the superior performance of \ourapproach.
    %\item We conduct a thorough evaluation of \ourapproach by comparing with three state-of-the-art optimization approaches: (i) \textsc{JUMBO}, (ii) \textsc{SMAC}, and (iii) \textsc{Unicorn} on three \textsc{MLperf} pipelines (object Detection, natural language processing, and speech recognition), a video analytics pipeline, and a database system by considering a range of different environmental changes. 
\end{itemize}
The artifacts and supplementary materials can be found at \href{https://github.com/anonpassen/CAMEO}{\color{blue!80} https://github.com/anonpassen/CAMEO}.
% We compare \ourapproach with state-of-the-art configuration optimization and ML-based performance debugging approaches. Overall, we find that \ourapproach is (at most) $13\times$ faster with $13\%$ better accuracy and $32\%$ higher gain than the next best ML-based approaches for single-objective faults. Compared to single-objective optimization approaches, \ourapproach can find repairs to misconfigurations $9\times$ faster while performing as well as (or better than) the best configuration discovered by the optimization techniques. Further, \ourapproach can find effective repairs for faults in multiple performance objectives (\ie, latency and energy consumption) with accuracy and gain as high as $16\%$ and $36\%$, respectively, than other ML-based performance debugging methods. Compared to multi-objective optimization approaches, \ourapproach can find repairs $5\times$ faster while having similar performance gain. Finally, with a case study, we demonstrate that \ourapproach finds $14\%$ better repairs than the experts' advice in 24 minutes.

% \ourapproach would alleviate developers' burden, it is important to develop better methods to \emph{identify the root cause} of non-functional faults and \emph{fix} them early and in a principled way.
% If the prescribed repairs do not result in satisfactory performance improvement, \ourapproach updates the causal model with new observations and repeats the above steps until the performance objective has been met. 

% Advise against the use of optimization:
%  - Don't want the global optima, but the original configuration with the smallest change to reach the performance objective. 
% - It does not give us any information on the underlying causality of the system. The explainability/expressiveness is lost -- we won't know how/why a certain change is useful. 
% Our work is tangentially related to other work on performance modeling and optimization of highly configurable systems using machine learning and optimization \cite{wu2015deep, yigitbasi2013towards, zhang2015performance,siegmund2015performance, nair2018faster, filieri2015automated, iqbal2020flexibo, jamshidi2016uncertainty}. These methods are designed as push-button solutions to offer a near-optimal configuration, they do not offer Here we essentially tackle a different problem---that of finding the root causes of an already observed non-functional fault and finding a fix for it instead of finding an optimization.

% , static and dynamic software analysis \cite{kim2013splat, meinicke2016essential, velez2019configcrusher, abal2018variability, nguyen2016igen}, or sampling techniques \cite{sarkar2015cost, siegmund2015performance, guo2013variability, jamshidi2018learning}.

% % \bi[leftmargin=*]
%     \noindent \textbf{Technique.} Our approach is the first to exploit causal inference and counterfactual reasoning to reason about the root causes for non-functional faults and offer repairs to fix them. 
%     % Our approach achieves this without actually performing any intervention (i.e., changing the configuration and deploying the system with the new configurations). This is unlike statistical debugging where we cannot reason about changes unless we have seen several failures to create discriminative models.

%     \noindent\textbf{Tool.} We propose \ourapproach, a fully automated performance debugging approach that localizes the root causes of non-functional faults and fixes them. We show that \ourapproach can handle faults in multiple performance objectives simultaneously. \ourapproach is quite robust in that it can accommodate changes to software properties such as varying workloads. %We can reuse \ourapproach to reason about non-functional faults in environments where we cannot collect new observations or we have only very few observational data. 

%     \noindent \textbf{Real-world Evaluation.} We evaluate \ourapproach with 5 real-world highly configurable systems and it was able to identify the root causes and explain how the root causes (configuration options and interactions) triggered the fault, much more accurately with much less false negative compared with statistical debugging and the most popular heuristic approach in practice.
% % \ei



% \red{  Optimization tells us to configure under a certain way until the budget is finished. Need to collect new data to refine our estimate (bayesian opt) }
% \red{Analytical models require understanding and modeling of the system internal, which is impossible or expensive + data}
\

% \red{In eqs.~\ref{eq:do} and~\ref{eq:ace}, $\mathbb{E}(Y~|~do(X=x))$ is \textit{not} the same as the ordinary conditional distribution $\mathbb{E}\left(Y~|~X=x\right)$. This is because $\mathbb{E}\left(Y~|~X=x\right)$ takes the original population, as is, and filters it gets the sub-population where $X=x$. If $X=x$ does not exist in the population, the value of $\mathbb{E}\left(Y~|~X=x\right)$ would be misleading. In contrast, $\mathbb{E}\left(Y~|~\mathit{do}\left(X=x\right)\right)$ uses do-calculus rules~\cite{} to infer the value of distribution even when $X=x$ has never been encountered before. }



==> related_work.tex <==
\section{Related Work}
%In this section, we discuss some of the noteworthy literature related to \ourapproach.\\
\textbf{Performance Optimization in Configurable Systems.}
% Over the years, various methods have been tried to improve the functionality of configurable systems. 
Previous studies have demonstrated that misconfigurations often result in subpar system performance.~\cite{menon2020auto} proposed a framework HiPerBOt to determine application and platform-level configurations that give better system performance. To approximate the objective function and make Bayesian optimization scalable for numerous optimization options, BOCA~\cite{chen2021efficient} utilized a tree-based model and provided a searching strategy to make Bayesian optimization more efficient. By collecting system activity and transitioning from resource space to execution space for exploration, SCOPE~\cite{kim2022scope} optimizes the system objective and reduces safety constraint violations. Additionally, Cello~\cite{ding2022cello}, an optimization framework for systems proposed prediction-based early termination of sample collection by censored regression. However, above mentioned works do not incorporate the direct influence of configuration changes in the source and target environment and \ourapproach proposes an efficient optimization strategy focusing on the distribution shift of performance measures in the target environment due to such changes.
% HIRE~\cite{blocher2021switches} proposed a resource model for addressing heterogeneity, resource interchangeability, and non-linear resource requirements for performance optimization. 
 
% To identify system errors and assess the effects of various customizable parameters on system performance, prior works have used two types of approaches: static and dynamic program analysis.
% ~\cite{siegmund2015performance} presented a performance-influence model for configurable systems and illustrates the effects of various configurable parameters on system performance by combining binary and numerical configuration parameters using machine learning and sampling heuristics.
% ~\cite{temple2017learning} proposed a system to reduce the configuration search space by staging the configuration process and only permitting the configurations that satisfy the customer requirements of low latency or memory utilization.~\cite{guo2013variability} proposed a variability-aware approach to forecast system performance using a small sample of measured variants, statistical learning, and random sampling. In DECART~\cite{guo2018data}, a data-efficient learning method is introduced to predict system performance based on a small sample of system configurations. 


\textbf{Transfer Learning for Performance Modeling.}
Transferring performance behavior knowledge across different environments to optimize system configuration is advantageous.~\cite{jamshidi2017transfer} identified several prominent knowledge for transfer learning by varying software configurations and environmental variables.~\cite{iqbal_transfer_2019} examined various transfer learning strategies and utilized the most pertinent system configurations to generate optimized performance models for Deep Neural Network systems at a lower cost.~\cite{valov2020transferring} proposed a method for approximating and transferring the Pareto frontiers of optimal configurations across both homogeneous and heterogeneous hardware environments. In all this literature transfer learning is mainly focused on the source configurations rather than differences in target configurations and \ourapproach can address this gap. 
% to forecast the performance behavior of a target environment when configurations change and to reduce the size of the configuration space. 
% BEETLE~\cite{krishna2019whence}, identifies and studies the most pertinent source of historical data for optimized performance modeling.

% ~\cite{ballesteros2021transfer} used transfer learning to generate effective run-time quasi-optimal configurations of Dynamic Software Product Lines for performance models and prepared the initial population of Multi-Objectives Evolutionary Algorithms with the help of good configurations from similar systems and proposed a set of run-time optimization criteria for Cyber-Physical Systems vendors.

% A deep transfer learning network is generated by integrating the convolutional neural network and several domain adaption techniques in~\cite{li2020transfer}, where deep neural networks are trained using simulated data, and transfer learning reduces discrepancies caused by the model-process mismatch. 

\textbf{Usage of Causal Analysis in Configurable Systems.}
Causal analysis is used for different system optimization and debugging tasks in Configurable Systems.~\cite{fariha2020causality} points out the root causes of intermittent failures in software leveraging fault injection procedure.~\cite{johnson2020causal} suggested a method for analyzing and fixing software bugs by identifying a set of executions that make use of counterfactual causality theory and contain important causal information. To identify the true causes of bugs efficiently, they modify various inputs to the system while monitoring changes in system behavior. To identify the causes, effects, and interconnections of various causal aspects of configurable systems~\cite{dubslaff2022causality} suggested feasible algorithms. The advantage of \ourapproach over the above strategies is that the causality analysis in such works is solely based on the source environment however, \ourapproach combines attributes of both source and target environment to find true causes that drive the distribution shift in performance in the target environment.
% Furthermore, ConfigCrusher~\cite{VJSSAK:ASE20} uses static data-flow analysis, a white-box model, and the system's inbuilt implementation to evaluate system performance, extract different customizable system insights, and direct the performance study. 

% ~\cite{lemeire2007causal} evaluated the advantages of a dependency analysis and the decompositional capabilities of causal models to investigate the potential usage of causal modeling with the aid of the form-free information-theoretic concept of different mutual information. 


==> related_work_backup.tex <==
\section{Additional Related Work}
%In this section, we discuss different directions of related work in addition to those mentioned in \Cref{sec:intro}.\\
% In addition to all comments that I put in several previous versions, we need to have the sampling methods in the table and also clarifying guarantees in a new column.
% Applications such as hyperparameter tuning and the scale of the search space.
\textbf{Performance Optimization in Configurable Systems.}
%A large body of performance optimization methods have been proposed to improve the functionality of configurable systems. 
BO based optimization methods are used to discover the best configuration suited for a particular application and platform \cite{menon2020auto} and to streamline compiler autotuning \cite{chen2021efficient}. SCOPE~\cite{kim2022scope} improves system performance and lowers safety constraint breaches by gathering system activity and switching from resource space to execution space for exploration. \cello~\cite{ding2022cello} uses prediction-based early termination of sample collection by censored regression. Siegmund et al.~\cite{siegmund2015performance} proposed a performance-influence model for configurable systems to understand the influence of configuration options on system performance using machine learning and sampling heuristics. Nevertheless, these techniques are platform specific and are not suitable when a performance distribution shift occurs due to environmental changes. In comparison, \ourapproach tackles the shift by transferring causal knowledge using causal performance models.
% Earlier studies have demonstrated that misconfigurations often result in subpar system performance.
% To identify system errors and assess the effects of various customizable parameters on system performance, prior works have used two types of approaches: static and dynamic program analysis.
% In order to find optimal application and platform-level system configuration~\cite{menon2020auto} proposed a framework HiPerBOt. Moreover, as Bayesian optimization techniques are utilized many a times for generating system configuration with better system performance, BOCA~\cite{chen2021efficient} utilized a tree-based model and provided a searching strategy to make them more efficient by approximating the objective function and making Bayesian optimization more scalable.
% \\
% Furthermore, heterogeneity, resource interchangeability, and non-linear resource requirements of deployed models in a system play important role in performance optimization and therefore, HIRE~\cite{blocher2021switches} proposed a resource model to satisfy above requirements. 
 
% However, exploration space of available parameters is often too large and hence~\cite{temple2017learning} reduces the configuration search space by staging the configuration process and only permitting the configurations that satisfy the customer requirements of low latency or memory utilization.
% Besides, statistical techniques are often utilized to predict system behaviour.~\cite{guo2013variability} proposed CART, a variability-aware approach to forecast system performance using a small sample of measured variants, statistical learning, and random sampling. Moreover, in DECART~\cite{guo2018data}, a data-efficient learning method is introduced to predict system performance based on a small sample of system configurations. \\

% \textsc{ResTune}~trains an ensemble model to represent prior knowledge from historical tasks and uses it to help reduce the tuning time for the target task via a meta-learning based approach.
 
\noindent \textbf{Transfer Learning for Performance Modeling.}
It is possible to expedite the optimization process by transferring performance behavior knowledge from one environment to another. However, it is essential to identify which knowledge is necessary to be transferred to reach this aim. Jamshidi et al.~\cite{jamshidi2017transfer} showed that when the environment changes are small, knowledge for forecasting performance can be transferred, while only knowledge for efficient sampling can be transferred when the environment changes are severe. Krishna et al.~\cite{krishna2019whence}determined the most relevant source of historical data to optimize performance modeling. Valov et al.~\cite{valov2020transferring} proposed a novel method for approximating and transferring the Pareto frontiers of optimal configurations across different hardware environments. Ballesteros et all.\cite{ballesteros2021transfer} proposed a transfer learning assisted dynamic evolutionary algorithm to generate effective run-time quasi-optimal configurations of Dynamic Software Product Lines. All these techniques incorporate transfer learning based on correlational statistics (ML-based). However, \Cref{sec:motivation_causal} shows that ML-based models are prone to capturing spurious correlations. In comparison, \ourapproach makes use of causal-based models, which identify invariant features despite environmental fluctuations.
%and prepared the initial population of Multi-Objectives Evolutionary Algorithms with the help of good configurations from similar systems, and proposed a set of run-time optimization criteria for Cyber-Physical Systems vendors.
% Besides traditional transfer learning techniques,~\cite{li2020transfer} generated a deep transfer learning network by integrating the convolutional neural network and several domain adaption techniques, where deep neural networks are trained using simulated data, and transfer learning reduces discrepancies caused by the model-process mismatch.


\noindent \textbf{Usage of Causal Analysis in Configurable Systems.}
Causal analysis has been used for various debugging and optimization tasks in configurable systems. 
% For example, AID~\cite{fariha2020causality} and ~\cite{johnson2020causal} introduced approaches to facilitate the software debugging procedure.
Fariha et al.\cite{fariha2020causality} proposed AID which conducts intervention through fault injection to pinpoint the root cause of intermittent failures in software. Johnson et all.\cite{johnson2020causal} proposed Causal Testing to analyze and fix software bugs by identifying a set of executions that contain important causal information. Causal analysis can further be helpful for measuring the system performance and provide notable insights to determine the optimal setting for the systems. Dubslaff et all.\cite{dubslaff2022causality} defined a notion of feature cause, proposed a method to effectively compute feature causes and causal explications, and leveraged the feature causes to facilitate root cause identification, and feature effect / interaction estimation. The causality analysis in these works is solely based on one environment. In contrast, our studied problem involves two environments (source and target). As shown in \Cref{sec:motivation_causal_in_various_environments}, some differences can exist between causal structures of the two environments so the approaches in the aforementioned work cannot be applied in our setting. Our proposed \ourapproach addresses the issue by training two causal based models for source and target respectively and leverage both during the configuration optimization process.
